WritePolicyBench: Benchmarking Memory Write Policies under Byte Budgets

We introduce WritePolicyBench, a benchmark for evaluating memory write policies: decision rules that choose what to store, merge, and evict under a strict byte budget while processing a stream with document/API drift. The benchmark provides (i) task generators with controlled non-stationarity, (ii) an explicit action interface for external memory, (iii) a byte-accurate cost model, and (iv) standardized metrics that measure both task success and budget efficiency.

==> sections/00_abstract.tex <==
WritePolicyBench is a benchmark for evaluating \emph{memory write policies}: decision rules that choose what to store in a bounded memory when processing a stream of observations under a strict byte budget. The benchmark focuses on synthetic task streams with controlled distribution drift regimes (e.g., bursty changes and redundancy) and a simple memory interface that exposes explicit write actions. We provide baseline policies (e.g., FIFO store-all, last-$k$ bytes, and no-memory) and standardized metrics that measure both task success and budget efficiency. The benchmark is intended to support controlled ablations and reproducible comparisons of write-policy behavior.
